Grid-Centric Traffic Scenario Perception for Autonomous Driving: A Comprehensive Review

Grid-centric perception is a crucial field for mobile robot perception and navigation. Nonetheless, grid-centric perception is less prevalent than object-centric perception as autonomous vehicles need to accurately perceive highly dynamic, large-scale traffic scenarios and the complexity and computational costs of grid-centric perception are high. In recent years, the rapid development of deep learning techniques and hardware provides fresh insights into the evolution of grid-centric perception. The fundamental difference between grid-centric and object-centric pipeline lies in that grid-centric perception follows a geometry-first paradigm which is more robust to the open-world driving scenarios with endless long-tailed semantically-unknown obstacles. Recent researches demonstrate the great advantages of grid-centric perception, such as comprehensive fine-grained environmental representation, greater robustness to occlusion and irregular shaped objects, better ground estimation, and safer planning policies. There is also a growing trend that the capacity of occupancy networks are greatly expanded to 4D scene perception and prediction and latest techniques are highly related to new research topics such as 4D occupancy forecasting, generative AI and world models in the field of autonomous driving. Given the lack of current surveys for this rapidly expanding field, we present a hierarchically-structured review of grid-centric perception for autonomous vehicles. We organize previous and current knowledge of occupancy grid techniques along the main vein from 2D BEV grids to 3D occupancy to 4D occupancy forecasting. We additionally summarize label-efficient occupancy learning and the role of grid-centric perception in driving systems. Lastly, we present a summary of the current research trend and provide future outlooks.

==> contents/notused_2-bev2d.tex <==
\section{Bird's-Eye View 2D Grid Representation}\label{sec:BEVRepre}
BEV grid is a common representation of obstacle detection for on-road vehicles. The basic technique for grid-centric perception is to map raw sensor information to BEV grid cells, which differ in mechanisms for different sensor modalities. LiDAR point clouds are naturally represented in 3D space, so there is a long-standing tradition of extracting point or voxel features on BEV maps\cite{PointRCNN,PV-RCNN}. Cameras are rich in semantic cues but lack geometric cues, which makes 3D reconstruction an ill-posed problem. The rising Vision BEV perception casts new lights on view transformation between perspective view to bird's eye view (PV2BEV).



\subsection{LiDAR-based Grid Mapping}\label{sec:lidar2bev}
Feature extraction of LiDAR point clouds follows the following paradigms: point, voxel, pillar, range view, or hybrid feature from above\cite{3DODSurvey}. This section focuses on the feature mapping of point clouds to BEV grids. 

LiDAR data collected in 3D space can be easily transformed to BEV and fused with information from multi-view cameras. The sparse and variable density of LiDAR point clouds renders CNNs inefficient. Some methods \cite{MV3D,AVOD,PIXOR} voxelize the point cloud into a uniform grid and encode each grid cell with hand-crafted features. MV3D\cite{MV3D}, AVOD\cite{AVOD} generates the BEV representation by encoding each grid with height, intensity, and density features. BEV representation in PIXOR\cite{PIXOR} is a combination of the 3D occupancy tensor and the 2D reflectance map, which keep the height information as channels. BEVDetNet\cite{BEVDetNet} further reduces BEV-based model latency to 2ms on Nvidia Xavier embedded platform. For advanced temporal tasks on grids, MotionNet proposes a novel spatial-temporal encoder STPN\cite{MotionNet} which aligns past point clouds to the current ego pose. The network design is shown in Fig. \ref{motionnet_stpn}. 

However, these fixed encoders are not successful in utilizing all the information contained within the point cloud. The learned features become a trend. VoxelNet\cite{VoxelNet} stacks voxel feature encoding (VFE) layers to encode point interactions within a voxel and generates a sparse 4D voxel-wise feature. And then VoxelNet uses a 3D convolutional middle layer to aggregate and reshape this feature and passes it through a 2D detection architecture. To avoid hardware-unfriendly 3D convolution, the pillar-based encoder in PointPillars\cite{PointPillars} and EfficientPillarNet\cite{efficientpillarnet} learns features on pillars of the point cloud. The features can be scattered back to the original pillar positions to generate a 2D pseudo-image. PillarNet\cite{PillarNet} further develops pillar representation by fusing densified pillar semantic features with spatial features in the neck module for final detection with orientation-decoupled IoU regression loss. The encoder for PillarNet\cite{PillarNet} is illustrated in Fig. \ref{pillarnet_pipeline}.

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.45\textwidth]{fig/pillarnet_pipeline.jpg}
	\caption{PillarNet\cite{PillarNet}: The pillar-based encoder proposed in PillarNet achieves state-of-the-art performance as well as super fast computation.}
	\label{pillarnet_pipeline}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.3\textwidth]{fig/motionnet_stpn.jpg}
	\caption{STPN\cite{MotionNet}: Spatial-temporal encoder which extracts multi-frame voxel features using only 2D CNN blocks, used in \cite{MotionNet,MotionSC,LiCaNet,LiCaNeXt}}
	\label{motionnet_stpn}
\end{figure}


\subsection{Camera-based Grid Mapping}\label{sec:pv2bev}
As cameras provide information rich in semantic cues but lossy in geometric cues. Early researchers conduct 3D vision tasks on the perspective view (PV), which lacks enough geometry guidance. In recent years, vision BEV-based approaches achieve great success as BEV provides a structured coordinate encoding for pixel features from multi-view cameras. View projection from perspective view (PV) to bird's eye view (BEV) is a major issue for vision-centric grid perception. In this section, we focus on dense BEV mapping approaches rather than sparse-query-based representation\cite{StreamPETR, Sparse4D}. 


\subsubsection{Geometry-based View Transformation}\label{sec:geo-pv2bev}
Geometry-based methods utilize the natural geometric projection relationship between PV and BEV for transformation. These methods can be further divided into two categories: homograph-based and depth-based.  Homograph-based methods are efficient for learning road surface layouts for autonomous driving, due to their hard flat-ground assumption. Depth-based methods are more common in representing obstacles on the road and achieving state-of-the-art performance.

\textbf{Homograph-based methods.} Inverse Perspective Mapping (IPM)\cite{IPM} is the earliest and the most important work which uses a homography matrix to formulate the transformation under the constraint that the corresponding points lie on a horizontal plane. The homography matrix can be mathematically derived from intrinsic and extrinsic parameters of the camera. In addition to image projection, Cam2BEV\cite{Cam2BEV}, 3D-LaneNet\cite{3D-LaneNet} use IPM to transform feature maps for downstream perception tasks. Gu et al.\cite{HomoLoss} propose a Homography Loss for the training of the network. To reduce the distortion of the part above the ground plane caused by IPM, OGMs\cite{OGMs}, SHOT\cite{SHOT} use semantic information and MonoLayout\cite{MonoLayout} utilizes Generative Adversarial Network (GAN)\cite{GAN} to improve BEV features.


\textbf{Depth-based methods.} These methods rely heavily on voxels, an explicit 3D representation compatible with the end-to-end design. As shown in Fig. \ref{lss_depthnet}, depth-based methods use the predicted depth distribution per grid to lift 2D features to 3D voxel space and then generate the BEV 2D grid representation. This lift process writes:
\begin{equation}
	\mathcal{F}_{3D}(x,y,z)=[\mathcal{F}^{*}_{2D}(u,v)\otimes \mathcal{D}^{*}(u,v)  ]_{x,y,z},
\end{equation}
where $(u,v)$ is pixel coordinate corresponding to $(x,y,z)$ in 3D space, $\mathcal{F}$ is feature, $\mathcal{D}$ is predicted depth distribution, * denotes one or more images, $\otimes$ denotes outer production. 

Depth is commonly formulated as a distribution. OFT\cite{OFT}, M2BEV\cite{M2BEV} assume uniform depth distribution, which means that all 3D features along a ray are the same. Some other depth-based methods\cite{CaDDN,DfM,LSS,BEVDepth,STS,MV-FCOS3D++} model the depth distribution with different learnable network structures and parameters.

Depth-based methods are usually supervised by labels from downstream tasks, but per-pixel depth supervision can also improve accuracy of depth estimation. CaDDN\cite{CaDDN}, DfM\cite{DfM}, BEVDepth\cite{BEVDepth} and STS\cite{STS} can optionally use depth supervision from LiDAR point clouds during the training stage. 

Some structures are able to capture stereo cues in ring-camera settings. MV-FCOS3D++\cite{MV-FCOS3D++} uses pre-trained 2D feature extractors for a few stereo cues. BEVDepth proposes a depth correction module to solve the spatial misalignment between the image feature map and the ground truth derived from LiDAR caused by the ego vehicle's motion. Combined with the monocular depth module in BEVDepth, BEVStereo\cite{STS} uses the geometrical correspondence between temporal dynamic stereo cameras to promote depth learning. 

Depth-based methods are still dominant in vision-centric perception. Recent works such as FIERY\cite{FIERY}, M2BEV\cite{M2BEV}, StretchBEV\cite{StretchBEV} and BEVerse\cite{BEVerse} are based on BEV representation derived from depth-based LSS\cite{LSS}.

\textbf{Fisheye BEV algorithm.} Compared to pinhole cameras, fisheye cameras have a broader field of view and higher distortion. Most fisheye detection algorithms are based on the perspective view. Wu et al.\cite{FPD_FPNet_TIV} propose a surround-view fisheye dataset FPD and BEV-perception multi-task model, FPNet. It has a shared feature extractor as well as 2D and 3D detection heads and per-pixel depth head.

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.45\textwidth]{fig/lss_depthnet.jpg}
	\caption{LSS\cite{LSS}: Probabilistic depth estimation in unprojecting images to BEV space, used in \cite{BEVDet,BEVDet4D,BEVerse,BEVFusion,BEVFusion2}}
	\label{lss_depthnet}
\end{figure}

% \begin{figure}[ht!]
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{fig/bevdepth_depthnet.jpg}
% 	\caption{BEVDepth\cite{MotionNet}: Depth estimation module which considers context information in BEVDepth}
% 	\label{bevdepth_depthnet}
% \end{figure}



\subsubsection{Network-based View Transformation}\label{sec:neural-pv2bev}

Network-based transformation methods utilize deep neural networks as a mapping function to model the view transformation and use the camera geometry implicitly. Recent methods can also be further divided into two categories: MLP-based and transformer-based. The former conducts the transformation in a forward way, while the latter constructs BEV queries and searches for corresponding features on PV maps through a cross-attention mechanism.

\textbf{MLP-based methods.} Multi-layer perceptron is employed to model the transformation from PV to BEV without camera parameters. Therefore, they avoid inductive biases from the calibrated camera system. VED\cite{VED} utilizes a variational encoder-decoder MLP network to predict BEV semantic occupancy grid map from a front-view monocular image in real-time. To use the information from different views to achieve surrounding sensing, VPN\cite{VPN} designs a view transformer module (VTM) with two-layer MLP to fuse each PV feature map into a BEV feature map. FishingNet\cite{FishingNet} transforms the camera features to BEV maps by modifying the VTM, and then fuse them with radar and LiDAR data for multi-modal perception and prediction. To predict more accurate BEV maps from monocular images, PON\cite{PON} and STA-ST\cite{STA-ST} include a feature pyramid network (FPN)\cite{FPN} to provide high-resolution features with rich context. The dense transformer layer in PON collapses PV features along height axis and expands them along the depth axis through MLP before resampling them to obtain BEV features in Cartesian coordinates. HDMapNet\cite{HDMapNet} puts forward a novel view transformer module that consists of MLP-based neural feature transformation and geometric projection. It can produce a vectorized local semantic map from images of the surrounding cameras. Since the projection of BEV features back to the PV map can form self-supervision, PYVA\cite{PYVA} includes a cross-view transformation module that utilizes an MLP-based cycle to retain the features related to view transformation. To reap the benefits of homograph-based methods and MLP-based methods, HFT\cite{HFT} consists of two branches to utilize geometric priors and global context respectively.

MLP-based methods tend to transform multi-view images individually and ignore the geometric potential brought by overlapping regions. These shortcomings make its application less widespread than subsequent transformer-based methods.

\textbf{Transformer-based methods.} Vaswani et al.\cite{Transformer} introduce transformer, an attention-based model which facilitates the development of natural language processing (NLP). Vision transformers have shown remarkable performance in various vision tasks due to its ability to capture long-range dependencies and global receptive fields. Compared to MLP-based methods, transformer-based methods view transformation have more impressive PV2BEV relation modeling ability. Query-based element extraction starts with 2D object detector DETR\cite{DETR}. 

To satisfy the requirements of grid-centric perception tasks, the granularity of the query in the transformer decoder should be finer and each query is position-encoded according to its spatial location in 3D space or BEV space. Tesla\cite{Tesla} first conducts the view transformation through cross-attention between dense BEV queries and multi-view image features. CVT\cite{CVT} points out that geometric reasoning of cross-attention transformers performs well and inferences faster than geometric models. So it employs cross-view transformers for view transformation, which use positional embeddings derived from calibrated camera intrinsics and extrinsics. In addition to an MLP-based cycled view projection mentioned above, PYVA's\cite{PYVA} transformation module also contains a cross-view transformer to correlate the features before and after view projection.

To avoid high computation complexity in the transformer attention module, one approach is to use sparse attention. Deformable attention\cite{DeformableAttention} reduces the number of keys to avoid excessive attention computation by only focusing on relevant regions and capturing informative features. The view transformation module of many works use this sparse attention, such as BEVSegFormer\cite{BEVSegFormer} shown in Fig. \ref{bevsegformer_pipeline}, PersFormer\cite{PersFormer} and BEVFormer\cite{BEVFormer}. Note that the queries in BEVSegFormer directly predict the reference points on images, while PersFormer and BEVFormer rely on camera parameters to compute the reference points. Apart from deformable attention, several kinds of sparse attention are put forward. GKT\cite{GKT} unfolds kernel regions around the projected reference points and makes them interact with dense BEV queries to generate BEV representation. ViT-BEVSeg\cite{ViT-BEVSeg} uses simpler and plain vision transformer for patch embedding-based view transformation.

Another approach is to simplify the cross-attention computation with 3D geometry constraints. Image2Map\cite{Image2Map} uses camera geometry to dictate one-to-one correspondence between vertical scan lines in the image and polar rays in the BEV map to form an inter-plane attention mechanism. The view transformation is treated as a set of sequence-to-sequence translations. Similarly, PolarFormer\cite{PolarFormer} also employs this correspondence to simplify the global attention into column-wise attention and uses a polar alignment module to aggregate rays from multiple camera views to generate a structured Polar BEV feature map.

PETRv2\cite{PETRv2} is developed from PETR\cite{PETR} which contains sparse object queries for object-centric tasks. In order to form a unified framework for 3D perception, PETRv2 adds a set of BEV segmentation queries to support high-quality BEV segmentation, an important grid-centric task.

Geometric cues and temporal cues are both important to transformer-based methods. As geometric cues, calibrated camera parameters are utilized in many transformer-based methods to reduce memory/computation complexity or improve data efficiency. As mentioned above, \cite{CVT,PETRv2} generate 3D positional embedding derived from camera parameters to help the transformers learn view transformation. \cite{PersFormer,BEVFormer,GKT} rely on camera parameters to compute the reference points for feature sampling. \cite{Image2Map,PolarFormer} employs camera geometry to dictate the relationship between each vertical scanline in the image and the BEV features. However, with such geometric cues it is possible to introduce inductive biases contained in the calibrated camera system. Temporal cues which are used in \cite{BEVFormer,PolarFormer} can improve the performance of methods.

\textbf{Polar coordinate.} Common practices adopt Cartesian coordinate with evenly distributed rectangular grids. However, PolarBEV\cite{PolarBEV} argues that surrounding grids should be paid more attention than distant ones, so unevenly distributed polar rasterization can reduce computational budget. PolarDETR\cite{PolarDETR} models multi-view BEV detection transformer on Polar parameterizations. PolarFormer\cite{PolarFormer} extracts dense BEV features on polar coordinates and surpasses Cartesian coordinate counterparts in BEVFormer\cite{BEVFormer}. 

\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.45\textwidth]{fig/bevsegformer_pipeline.jpg}
	\caption{BEVSegFormer\cite{BEVSegFormer}: The transformer-based BEV segmentation model introduced in BEVSegFormer.}
	\label{bevsegformer_pipeline}
\end{figure}

\subsection{Deep Fusion on Grids}\label{sec:deepfusion}

Multi-sensor multi-modality fusion has been a long-standing issue for automotive perception. Fusion frameworks are often categorized into early fusion, deep fusion, and late fusion. Among them, deep fusion has demonstrated the best performance in an end-to-end framework. Grid-centric representation serves as a unified feature embedding space for deep fusion among multiple sensors and agents.

\subsubsection{Multi-sensor Fusion}\label{sec:multisensorfusion}
Different sensors are inherently complementary: Cameras are geometry-loss but semantics rich, while LiDARs are semantics-loss but geometry rich. Radars are geometry and semantics sparse but robust to different weather conditions. Deep fusion fuses latent features across modalities and compensates for the limitations of each sensor. 

\textbf{LiDAR-camera fusion.} Some methods perform the fusion operation at a higher 3D level and support feature interaction in 3D space. UVTR\cite{UVTR} samples features from the image according to predicted depth scores and associates features of point clouds to voxels according to the accurate position. Thus, the voxel encoder for cross-modality interaction in voxel space can be introduced.  AutoAlign\cite{AutoAlign} designs a cross-attention feature alignment module (CAFA) to enable the voxelized feature of point clouds to perceive the whole image and perform feature aggregation. Instead of learning the alignment through the network in AutoAlign\cite{AutoAlign}, AutoAlignV2\cite{AutoAlignV2} includes a cross-domain DeformCAFA and employs the camera projection matrix to obtain the reference points in the image feature map. FUTR3D\cite{FUTR3D} and TransFusion\cite{Transfusion} fuses features based on attention mechanism and queries. FUTR3D employs a query-based modality-agnostic feature sampler(MAFS) to extract multi-modal features according to 3D reference points. TransFusion relies on LiDAR BEV features and image guidance to generate object queries and fuses these queries with image features. A simple and robust approach is to unify fusion on BEV features. Two implementations of BEVFusion\cite{BEVFusion,BEVFusion2}, shown in Fig. \ref{bevfusion_pipeline} unify features from multi-modal inputs in a shared BEV space. DeepInteration\cite{DeepInteration} and MSMDFusion\cite{MSMDFusion} designs multi-model interaction in BEV space and voxel space to better align spatial features from different sensors.



\begin{figure}[ht!]
	\centering
	\includegraphics[width=0.45\textwidth]{fig/bevfusion_pipeline.jpg}
	\caption{BEVFusion\cite{BEVFusion}: A simple and unified BEV feature-level fusion framework for LiDARs, cameras and radar points.}
	\label{bevfusion_pipeline}
\end{figure}


\textbf{Camera-radar fusion.} Radar sensors are originally designed for Advanced Driving Assistance System (ADAS) tasks, so their accuracy and density are insufficient for use in high-level autonomous driving tasks. OccupancyNet\cite{OccupancyNet} and NVRadarNet\cite{NVRadarNet} only use radars to perform real-time obstacle and free space detection. Camera-radar fusion is a promising low-cost perception solution that supplements semantics to radar geometry. Simple-BEV\cite{Simple-BEV}, RCBEVDet\cite{RCBEVDet}, and CramNet\cite{CramNet} have investigated different approaches for radar feature expression on BEV and fusion with vision BEV features. RCBEVDet\cite{RCBEVDet} process the multi-frame aggregated radar point clouds with a PointNet++\cite{PointNet++} network. CramNet\cite{CramNet} sets the camera features as query and radar features as value to retrieve radar features along the pixel ray in 3D space. Simple-BEV\cite{Simple-BEV} voxelizes multi-frame radar point clouds as a binary occupancy image and uses meta-data as additional channels. RRF\cite{RRF} yields a 3D feature volume from each camera by projection and sampling and then concatenates a rasterized radar BEV map. It finally gets a BEV feature map by reducing the vertical dimension.

\textbf{Lidar-camera-radar fusion.} LiDAR, radar, and camera fusion is a robust fusion strategy for all weathers. RaLiBEV\cite{RaLiBEV} adopts an interactive transformer-based bev fusion that fuses LiDAR point clouds and radar range azimuth heatmaps. FishingNet\cite{FishingNet} uses top-down semantic grids as a common output interface to conduct late fusion of the LiDAR, radars and cameras and performs short-term prediction of semantic grids. 

\subsubsection{Multi-agent Fusion}\label{sec:multiagentfusion}
Recent works on grid-centric perception are mostly based on single-agent systems, which have limitations in complex traffic scenes. Advancements in Vehicle-to-Vehicle(V2V) communication technologies enable vehicles to share their sensory information. CoBEVT\cite{CoBEVT} is the first multi-agent multi-camera perception framework that can generate BEV segmented maps cooperatively. In this framework, the ego vehicle geometrically warps the received BEV features according to the pose of the sender and then fuses them using a transformer with fused axial attention (FAX). Dynamic occupancy grid map (DOGM) also shows the capacity of reducing uncertainty in the fusion platform for multi-vehicle cooperative perception\cite{CoopDOGM,MVMS-OGM, GevBEV}.



==> contents/taxonomy.tex <==
\begin{figure*}[htbp]
 \centering
\begin{forest}
  forked edges,
  for tree={
    grow=east,
    reversed=true,%increase counter-clockwise
    anchor=base west,
    parent anchor=east,
    child anchor=west,
    base=left,
    font=\small,
    rectangle,
    draw={hiddendraw, line width=0.6pt},
    rounded corners,align=left,
    minimum width=2.5em,
    edge={black, line width=0.55pt},
    l+=1.9mm,
    s sep=7pt,
    inner xsep=7pt,
    inner ysep=8pt,
    ver/.style={rotate=90, rectangle, draw=none, rounded corners=3mm, fill=red, text centered,  text=white, child anchor=north, parent anchor=south, anchor=center, font=\fontsize{10}{10}\selectfont,},
    level2/.style={rectangle, draw=none, fill=orange,  
    text centered, anchor=west, text=white, font=\fontsize{8}{8}\selectfont, text width = 7em},
    level3/.style={rectangle, draw=none, fill=brown,   fill opacity=0.8,text centered, anchor=west, text=white, font=\fontsize{8}{8}\selectfont, text width = 2.7cm, align=center},
    level3_2/.style={rectangle, draw=none, fill=gray,   fill opacity=0.8,text centered, anchor=west, text=white, font=\fontsize{8}{8}\selectfont, text width = 2.7cm, align=center},
    level3_1/.style={rectangle, draw=none, fill=brown,   fill opacity=0.8, text centered, anchor=west, text=white, font=\fontsize{8}{8}\selectfont, text width = 3.2cm, align=center},
    level4/.style={rectangle, draw=red, text centered, anchor=west, text=black, font=\fontsize{8}{8}\selectfont, align=center, text width = 2.9cm},
    level5/.style={rectangle, draw=red, text centered, anchor=west, text=black, font=\fontsize{8}{8}\selectfont, align=center, text width = 14.7em},
    level5_1/.style={rectangle, draw=red, text centered, anchor=west, text=black, font=\fontsize{8}{8}\selectfont, align=center, text width = 26.1em},
    level5_2/.style={rectangle, draw=red, text centered, anchor=west, text=black, font=\fontsize{8}{8}\selectfont, align=center, text width = 30.0em},
    level5_3/.style={rectangle, draw=red, text centered, anchor=west, text=black, font=\fontsize{8}{8}\selectfont, align=center, text width = 35.0em},
  },
  where level=1{text width=5em,font=\scriptsize,align=center}{},
  where level=2{text width=6em,font=\tiny,}{},
  where level=3{text width=6em,font=\tiny}{},%yshift=0.26pt
  where level=4{text width=5em,font=\tiny}{},%yshift=0.26pt
  where level=5{font=\tiny}{},%yshift=0.26pt
  [Grid-centric perception, ver
 %    [OGM fundamentals 
 % \\(Sec. \ref{appendix:ogm} ), level2  [Occupancy grid map (Sec. \ref{appendix:ogm_base}){;} Continuous grid map (Sec. \ref{appendix:com}) {;} Dynamic grid map (Sec. \ref{appendix:dogm}) , level5_3]]
 %    [BEV 2D grid \\
 % (Sec. \ref{sec:BEVRepre}), level2
 %        [LiDAR BEV (Sec. \ref{sec:lidar2bev}), level3
 %        ]
 %        [Vision BEV (Sec. \ref{sec:pv2bev}), level3
 %            [Geometry-based PV2BEV (Sec. \ref{sec:geo-pv2bev}){;} Network-based PV2BEV (Sec. \ref{sec:neural-pv2bev}) , level5_1]
 %        ]
 %        [Fusion (Sec. \ref{sec:deepfusion}), level3
 %            [Multi-sensor fusion (Sec. \ref{sec:multisensorfusion}){;} Multi-agent fusion (Sec. \ref{sec:multiagentfusion}) , level5_1]
 %        ]]
     [OGM fundamentals 
 \\(Sec. A ), level2  [Occupancy grid map (Sec. A2){;} Continuous grid map (Sec. A3) {;} Dynamic grid map (Sec. A4) {;} Memory-efficient 3D mapping , level5_3]]
       [BEV 2D grid \\
 (Sec. B\&C), level2 [LiDAR BEV (Sec. B1) {;} Vision BEV (Sec. B2) {;} Fusion on grids (Sec. B3) {;} Perception tasks (Sec. C) , level5_3]
 ]
        [3D occupancy \\
 (Sec. \ref{sec:3d_occu}), level2
        [LiDAR SSC (Sec: \ref{sec:lidarssc}), level3
        ]
        [Vision 3D (Sec: \ref{sec:visionssc}), level3
            [Explicit voxel reconstruction (Sec. \ref{sec:exp-visionssc}){;} Implicit neural rendering (Sec. \ref{sec:imp-visionssc}) , level5_1]
        ]]
    [Temporal tasks
 \\(Sec. \ref{sec:temporal} ), level2  [Temporal BEV fusion(Sec. \ref{sec:temporal_bev}){;} Short-term motion (Sec. \ref{sec:short-term-motion}) {;} Long-term occupancy flow (Sec. \ref{sec:occu_flow}) , level5_3]]
        [Efficient learning \\
 (Sec. \ref{sec:effilearn}), level2
        [multitasking (Sec: \ref{sec:multitasking}), level3
            [Joint BEV Seg\&Motion (Sec. \ref{sec:multitasking-segmotion}){;} Joint 3D Det\& BEV Seg (Sec. \ref{sec:multitasking-detseg}){;} \\More multitasking (Sec. \ref{sec:multitasking-more}), level5_1]
        ]
        [Label-efficient \\(Sec: \ref{sec:label-effi}), level3
        ]
        [Computation-efficient \\(Sec: \ref{sec:compute-effi}), level3
            [Memory-efficient (Sec. \ref{sec:memory-effi}){;} Efficient PV2BEV  (Sec. \ref{sec:pv2bev-effi}) , level5_1]
        ]]
            [Grid applications\\ in AD systems \\
 (Sec. \ref{sec:driveapplication}), level2
        [Industrial design \\(Sec: \ref{sec:industrial}), level3
        ]
        [Related perception tasks \\(Sec: \ref{sec:relatedtasks}), level3
            [SLAM (Sec. \ref{sec:slam}){;} Map element detection  (Sec. \ref{sec:mapdet}) , level5_1]
        ]
        [Grid-based Planning \\(Sec: \ref{sec:planning}), level3
            [Graph search (Sec. \ref{sec:planning-graph}){;} Collision detection  (Sec. \ref{sec:planning-collision}) \\States in RL (Sec. \ref{sec:planning-state_rl}){;} End-to-end planning  (Sec. \ref{sec:planning-e2e}) , level5_1]
        ]]
]
\end{forest}
\caption{Hierarchically-structured taxonomy of grid-centric perception for autonomous driving.}
\label{fig:taxonomy}
\end{figure*}
